SuGaR: Surface-Aligned Gaussian Splatting for Efficient 3D Mesh Reconstruction and High-Quality Mesh Rendering

We propose a method to allow precise and extremely fast mesh extraction from 3D Gaussian Splatting. Gaussian Splatting has recently become very popular as it yields realistic rendering while being significantly faster to train than NeRFs. It is however challenging to extract a mesh from the millions of tiny 3D gaussians as these gaussians tend to be unorganized after optimization and no method has been proposed so far. Our first key contribution is a regularization term that encourages the gaussians to align well with the surface of the scene. We then introduce a method that exploits this alignment to extract a mesh from the Gaussians using Poisson reconstruction, which is fast, scalable, and preserves details, in contrast to the Marching Cubes algorithm usually applied to extract meshes from Neural SDFs. Finally, we introduce an optional refinement strategy that binds gaussians to the surface of the mesh, and jointly optimizes these Gaussians and the mesh through Gaussian splatting rendering. This enables easy editing, sculpting, rigging, animating, compositing and relighting of the Gaussians using traditional softwares by manipulating the mesh instead of the gaussians themselves. Retrieving such an editable mesh for realistic rendering is done within minutes with our method, compared to hours with the state-of-the-art methods on neural SDFs, while providing a better rendering quality. Our project page is the following: https://anttwo.github.io/sugar/

==> figures/intro.tex <==
\begin{figure}
    \centering
    \begin{tabular}{cc}
    \hfill
    \includegraphics[trim={20.cm 0 20.cm 0},clip,width=0.45\linewidth]{images/gaussian_arrangement/gaussian_vanilla.png} & 
    \includegraphics[trim={20.cm 0 20.cm 0},clip,width=0.45\linewidth]{images/gaussian_arrangement/gaussian_aligned.png} \\
    % \includegraphics{} & \includegraphics{} \\
    \end{tabular}
    \caption{\textbf{TOP: Arrangement of the Gaussians (left:) without and (right:) with our regularization term. } Without regularization, the Gaussians have no special arrangement after optimization, which makes extracting a mesh very difficult. \textbf{BOTTOM: Extracting a mesh (left:)} Even with our regularization term, Marching Cubes fail to extract a mesh while our method (\textbf{right}) succeeds.}
    \label{fig:one}
\end{figure}

==> figures/intro2.tex <==
\begin{figure*}
    \centering

    % Without regularization
    \begin{subfigure}{0.48\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 14.cm 0},clip,height=0.28125\linewidth,width=\linewidth]{images/gaussian_arrangement/gaussian_vanilla.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/vanilla_mc_1.png}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.24\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/vanilla_our_extraction_1.png} 
    \end{subfigure}
    \hfill
    %
    % With our regularization term
    \begin{subfigure}{0.48\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 12.cm 0},clip,height=0.28125\linewidth,width=\linewidth]{images/gaussian_arrangement/gaussian_aligned.png}
    \caption{Closeup on 3D Gaussians located near a surface}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/mc_sugar_1.png}
    \caption{Marching Cubes~\cite{lorensen-1987-marchingcubes}}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.24\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/full_sugar_1.png}
    \caption{Our extraction method}
    \end{subfigure}
    %\hfill
    \caption{\textbf{Reconstructing a 3D scene with Gaussians (top:) without and (bottom:) with our regularization term.} 
    \textbf{(a) Arrangement of the Gaussians on a planar surface}. Without regularization, the Gaussians have no special arrangement after optimization, which makes extracting a mesh very difficult. 
    \textbf{(b): Extracting a mesh with Marching Cubes.} Without our regularization term, Marching Cubes fail to extract a mesh. With our regularization term, Marching Cubes are able to recover an extremely noisy mesh of the scene. However this mesh contains a lot of unnecessary triangles inside the geometry, due to the algorithm reconstructing non-visible parts of the Gaussians. Ultimately, reconstructing small Gaussians with Marching Cubes requires using a very fine 3D grid and results in a high memory footprint. 
    \textbf{(c): Extracting a mesh with our proposed method.} Our extraction method is able to reconstruct a 3D mesh even without our regularization term, showing its superiority over Marching Cubes in this context. Still, the mesh is noisy. By contrast, our full method succeeds in efficiently reconstructing a clean mesh without noise nor unnecessary triangles. \antoinermk{This figure is too big, right?}}
    \label{fig:one}
\end{figure*}

==> figures/intro3.tex <==
\begin{figure*}
    \centering

    % Loss ablation (Gaussian alignment)
    \begin{subfigure}{0.49\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/gaussian_arrangement/gaussian_vanilla.png}
    \caption*{(a) Loss from original Gaussian Splatting~\cite{kerbl3Dgaussians}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}    
    \hfill
    \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/gaussian_arrangement/gaussian_aligned.png}
    \caption*{(b) With our regularization term}
    \end{subfigure}
    %\hfill
    
    % Mesh extraction ablation
    \begin{subfigure}{0.49\linewidth}    
        \hfill
        \begin{subfigure}{0.49\linewidth}    
        \hfill
        \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/vanilla_mc_1.png}
        \caption*{(a-1) Marching Cubes~\cite{lorensen-1987-marchingcubes}}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}    
        \hfill
        \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/vanilla_our_extraction_1.png} 
        \caption*{(a-2) Our extraction method}
        \end{subfigure}
        \hfill
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}     
        \hfill
        \begin{subfigure}{0.49\linewidth}    
        \hfill
        \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/mc_sugar_1.png}
        \caption*{(b-1) Marching Cubes~\cite{lorensen-1987-marchingcubes}}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}    
        \hfill
        \includegraphics[trim={0.cm 0 0.cm 0},clip,width=\linewidth]{images/garden/normals/full_sugar_1.png}
        \caption*{(b-2) Our extraction method}
        \end{subfigure}
        \hfill
    \end{subfigure}
    \hfill
    \caption{\textbf{Reconstructing a 3D scene with Gaussians (left:) without and (right:) with our regularization term.} 
    \textbf{TOP: Arrangement of the Gaussians on the surface}. Without regularization, the Gaussians have no special arrangement after optimization, which makes extracting a mesh very difficult. 
    \textbf{BOTTOM: Extracting a mesh.} \textbf{(a-1):} Without our regularization term, Marching Cubes fail to extract a mesh. 
    \textbf{(a-2):} Our extraction method is able to reconstruct a 3D mesh without regularizing the Gaussian splatting, showing its superiority over Marching Cubes in this context. Still, the mesh is very noisy. 
    \textbf{(b-1):} With our regularization term, marching cubes is able to recover an extremely noisy mesh of the scene. However this mesh contains a lot of unnecessary triangles inside the geometry, due to the algorithm reconstructing non-visible parts of the Gaussians. Ultimately, reconstructing small Gaussians with Marching Cubes requires using a very fine 3D grid and results in a high memory footprint. \antoinermk{Maybe I'm saying too much here, I don't know}
    \textbf{(b-2)} On the contrary, our full method succeeds in efficiently reconstructing a clean mesh without noise nor unnecessary triangles.}
    \label{fig:one}
\end{figure*}

==> figures/render_and_mesh_comparison.tex <==
\begin{figure*}[t]
  \centering
   \begin{subfigure}{0.16\linewidth}
        \includegraphics[trim={9.5cm 0 10.5cm 0},clip, width=\linewidth]{images/garden/gt/DSC07996.JPG}%
        %\vspace{.1em}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        %\includegraphics[width=\linewidth]{images/refined_mesh_normals/kitchen_sdfestim02_level01_decim1000000_gaussians_img4_normals.PNG}%
        %\vspace{.1em}
        \caption{\centering Garden vase from Mip-NeRF360~\cite{barron2022mipnerf360}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.16\linewidth}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/vanilla_mc_1.png}%
        \vspace{.1em}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/vanilla_mc_2.png}%
        %\vspace{.1em}
        \caption{\centering Loss from~\cite{kerbl3Dgaussians} + Marching Cubes~\cite{lorensen-1987-marchingcubes}}
    \end{subfigure}
    \hfill
   \begin{subfigure}{0.16\linewidth}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/vanilla_poisson_1.png}%
        \vspace{.1em}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/vanilla_poisson_2.png}%
        %\vspace{.1em}
        \caption{\centering Loss from~\cite{kerbl3Dgaussians} + Poisson~\cite{kazhdan-2006-poissonsurfacereconstruction} on centers}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.16\linewidth}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/vanilla_our_extraction_1.png}%
        \vspace{.1em}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/vanilla_our_extraction_2.png}%
        %\vspace{.1em}
        \caption{\centering Loss from~\cite{kerbl3Dgaussians} + Our mesh extraction}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.16\linewidth}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/full_sugar_1.png}%
        \vspace{.1em}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/normals/full_sugar_2.png}%
        %\vspace{.1em}
        \caption{\centering Our loss + Our mesh extraction}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.16\linewidth}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/gaussian/garden_sugar_render_3.png}%
        \vspace{.1em}
        %\fbox{\rule{0pt}{0.5in} \rule{0.8\linewidth}{0pt}}
        \includegraphics[width=\linewidth]{images/garden/gaussian/garden_sugar_render_4.png}%
        %\vspace{.1em}
        \caption{\centering Our mesh with surface 3D Gaussians}
    \end{subfigure}
    \hfill
   \caption{\textbf{Rendering and Mesh comparison.} \todo{To do. We see that both our mesh extraction method and our loss increase drastically the quality of the mesh. Explain that we had to take a high resolution for making the marching cubes passing trough a decent number of Gaussians; But still, it doesn't work.}}
   \label{fig:wo_and_w_regularization}
\end{figure*}

==> sec/00_teaser_editing_on_page_two.tex <==
\begin{figure*}
\begin{tabular}{cc}
    \includegraphics[width=0.5\linewidth]{images/test2_mesh.png} &
    \includegraphics[width=0.5\linewidth]{images/test2.png} \\
\end{tabular}
    \caption{Our mesh extraction algorithm binds Gaussians to the mesh and one can sculpt, modify, pose, animate, and composite the extracted mesh to edit the Gaussian Splatting representation. This opens new possibilities for Computer Graphics.}    
\label{fig:teaser_editing}
\end{figure*}


==> sec/00_teaser_mesh_on_page_one.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\vspace{-0.8cm}
\begin{center}
    \captionsetup{type=figure}
    \begin{tabular}{cc}
        \includegraphics[width=0.47\linewidth]{images/garden/clean/full_sugar_2.png} &
        \includegraphics[width=0.47\linewidth]{images/kitchen/clean/full_sugar_2.png} \\
        \includegraphics[width=0.47\linewidth]{images/garden/gaussian/garden_sugar_render_2.png} &
        \includegraphics[width=0.47\linewidth]{images/kitchen/gaussian/kitchen_sugar_render_2_decim1000000.png}\\
    \end{tabular}
\end{center}
\vspace{-0.5cm}
\captionof{figure}{
We propose an algorithm to extract a highly detailed mesh from any 3D Gaussian Splatting scene~\cite{kerbl3Dgaussians} within minutes on a single GPU~(\textbf{top:} Renderings of our meshes without texture, \textbf{bottom:} Renderings of the meshes with bound Gaussians). As shown in Figure~2, the mesh also makes possible the edition of the 3D Gaussian Splatting scene.
}
\label{fig:teaser_mesh}
\vspace*{0.5cm}
}]
